Causal Modeling of Policy Interventions From Sequences of Treatments and Outcomes

A treatment policy defines when and what treatments are applied to affect some outcome of interest. Data-driven decision-making requires the ability to predict what happens if a policy is changed. Existing methods that predict how the outcome evolves under different scenarios assume that the tentative sequences of future treatments are fixed in advance, while in practice the treatments are determined stochastically by a policy and may depend, for example, on the efficiency of previous treatments. Therefore, the current methods are not applicable if the treatment policy is unknown or a counterfactual analysis is needed. To handle these limitations, we model the treatments and outcomes jointly in continuous time, by combining Gaussian processes and point processes. Our model enables the estimation of a treatment policy from observational sequences of treatments and outcomes, and it can predict the interventional and counterfactual progression of the outcome after an intervention on the treatment policy (in contrast with the causal effect of a single treatment). We show with real-world and semi-synthetic data on blood glucose progression that our method can answer causal queries more accurately than existing alternatives.

==> content_v1.tex <==
\begin{abstract}
A \emph{treatment policy} defines when and what treatments are applied to affect some outcome of interest. Data-driven decision-making requires the ability to predict \emph{what happens if a policy is changed}. Existing methods that predict how the outcome evolves under different scenarios assume that the tentative sequences of future treatments are fixed in advance, while in practice the treatments are determined stochastically by a policy and may depend, for example, on the efficiency of previous treatments. Therefore, the current methods are not applicable if the treatment policy is unknown or a counterfactual analysis is needed. To handle these limitations, we model the treatments and outcomes jointly in continuous time, by combining Gaussian processes and point processes. Our model enables the estimation of a treatment policy from observational sequences of treatments and outcomes, and it can predict the interventional and counterfactual progression of the outcome \emph{after an intervention on the treatment policy} (in contrast with the causal effect of a single treatment). We show with real-world and semi-synthetic data on blood glucose progression that our method can answer causal queries more accurately than existing alternatives.
\end{abstract}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/figure1_v9.pdf}
    \caption{\textbf{(a)} Sequential treatment--outcome data for patients {\color{blue} A} (top) and {\color{red} B} (bottom). Patients follow distinct policies {\color{blue} $\pi_A$} and {\color{red}$\pi_B$} in the observation period $[0,10]$, where patient {\color{blue}A} is treated more frequently. A treatment causes a (slightly delayed) increase or `bump' in the outcome.
    \textbf{(b, c)} We now focus on patient {\color{blue}A} and show outcome trajectory $f$ (top) and treatment intensity $\lambda$ (bottom) in dashed lines. The estimates based on the observational data are in {\color{blue}blue}.
    \textbf{(b)} The interventional query corresponds to how the outcome  trajectory of {\color{blue}A} will progress \emph{after} the observation period (shaded area) under a treatment intensity induced by a \emph{different} policy {\color{red}$\pi_B$}, shown in {\color{red}red}.
    \textbf{(c)} The counterfactual query corresponds to how the outcome trajectory of {\color{blue}A} \emph{would have} progressed if the policy in the observation period $[0, 10]$ had been set to {\color{red}$\pi_B$} instead. 
    The observational data and estimations are shown in the background, while the counterfactual data and predictions are shown in {\color{red}red}.
    Notice some of the observed treatments are kept as counterfactual treatments $\mathbf{a}_\textit{cf}$, where the counterfactual intensity $\lambda_\textit{cf}$ is higher than the observational intensity $\lambda_\textit{obs}$. Counterfactual treatments in turn affect the counterfactual trajectory $f_\textit{cf}$.}
    \label{fig:compare}
\end{figure*}

\section{Introduction}

What policy should we adopt? In healthcare, for example, we observe patients' physiological markers (\emph{outcomes}) that change over time. %
We want to (positively) affect these outcomes %
%
by actions (\emph{treatments}) such as doses of a medicine. Sequences of outcomes and treatments are recorded as a time series. %
A \emph{policy} dictates what actions to take and when. To improve our policies, we must be able to assess their consequences: What is the effect of a given policy? What will be the effect of a change to a different policy? What would have happened if a patient had followed a different treatment policy? These questions correspond to observational, interventional, and counterfactual queries, %
%
and answering them is crucial, especially in domains such as public health and healthcare, where quantifying risks and expectations accompanying a policy decision, as well as evaluating past policies, is essential \citep{schulam2017reliable,bica2020estimating,oberst2019counterfactual,tsirtsis2020decisions,tsirtsis2021counterfactual}. Answering the interventional and counterfactual queries requires modeling policy interventions using a \emph{causal} model.

%
%

%
We want to infer a causal model of recurrent treatments from sequential treatment--outcome data.
%
%
%
%
Such data are always created by some policy, which induces dependencies between past events and future treatments.
However, the policy itself is generally not recorded and may be known only implicitly from the observed distribution of treatments and outcomes. 
In epidemiology, this problem has been studied using linear models for discrete-time sequences \citep{robins1986new,robins2009estimation,taubman2009intervening,zhang2018comparing},
though these works are unable to capture non-linear, long-term dependencies in real-world, continuous-time treatment--outcome sequences \citep{bica2021real}. \looseness-1

To handle such complex, long-term dependencies, sequential treatment--outcome models based on Bayesian nonparametrics and neural networks have been proposed \citep{xu2016bayesian,schulam2017reliable,soleimani2017treatment,bica2020estimating,seedat2022continuous}. However, they neglect the policy-induced link between past events and future treatments, and their causal analyses are limited to estimating the impact of a fixed sequence of treatments set by hand or generated by a simplistic parametric model. Such models do not generalize beyond simulations to the analysis of realistic treatment policies in real-world applications. Recently, \citet{hua2021personalized} modeled treatments explicitly; however, they focused on optimizing treatment strategies instead of causal estimation and only considered a parametric model tailored for a particular application.

%
%

%
%

%

With an appropriate causal model, we can also evaluate treatment policies using counterfactual reasoning, which allows for learning from mistakes by considering alternative scenarios to past events \citep{epstude2008functional,oberst2019counterfactual}. This is not considered by most of the literature, which focuses on future outcome progression. One recent work \citep{noorbakhsh2021counterfactual} applies counterfactual reasoning to event data using a counterfactual temporal point process, but does not consider a treatment--outcome setup (for further related work, see \cref{sec:related_work}).

To address these limitations, we propose a joint treatment--outcome model to estimate treatment policies and treatment responses in continuous time. Our contributions are:

\textbf{Joint treatment--outcome model.} We combine a marked point process and a conditional Gaussian process (\textsc{Gp}). Our \emph{non-parametric} model can be learned from observational sequential treatment--outcome data (Fig. 1(a)) and can estimate future and counterfactual progression.

\textbf{Interventional and counterfactual queries of interventions on policies.} We show that an intervention on a treatment policy is equivalent to a sequence of stochastic interventions on treatments, which we can model with our joint model, and use this to answer interventional (Fig. 1(b)) and counterfactual queries (Fig. 1(c)).

\textbf{Counterfactual sampling of arbitrary point processes.} We extend the algorithm of \citet{noorbakhsh2021counterfactual} from Poisson processes (independent events) to arbitrary point processes, allowing events to depend on past events.

We fit our model to a real-world data set on blood glucose progression, and from this generate realistic semi-synthetic use cases, where we show that our model accurately answers interventional and counterfactual policy queries. %

\section{Preliminaries}

Our work builds on Gaussian processes (for more details see \citet{williams2006gaussian}), marked point processes (\cref{sec:markedpointprocesses}) and causal inference (\cref{sec:causalinference}).

\subsection{Marked Point Processes (\textsc{Mpp})}
\label{sec:markedpointprocesses}

A temporal point process is a stochastic process that models a set of ordered random points $\{t_i\}_{i=1}^N$ on an interval $[0,T]$
%
\citep{daley2003introduction,rasmussen2011temporal}. This process is uniquely determined by its conditional intensity function $\lambda^*(\tau) = \lambda(\tau \mid \mathcal{H}_{<\tau})$, where the star superscript ${}^*$ denotes dependence on the past history $\mathcal{H}_{<\tau}$. The intensity function describes the instantaneous rate, i.e., the expected number of events in an infinitesimal interval $[\tau, \tau+\D\tau)$.
%

When each event time $t_i$ is associated with additional information (`mark')  $m_i$, we model $\mathcal{D} = \{(t_i, m_i)\}_{i=1}^N$ with a marked point process (\textsc{Mpp}). For an \textsc{Mpp}, the conditional intensity function additionally includes the conditional mark probability $p^*(m \mid t)$: $\lambda^*(t, m) = \lambda^*(t) p^*(m \mid t)$. The likelihood of $ \mathcal{D}$ observed in the interval $[0,T]$ is given by\looseness-1
\begin{equation*}
    \label{eq:mpp_lik}
    p(\mathcal{D} \mid \lambda^*(t, m)) = \left( \prod_{i=1}^N \lambda^*(t_i) p^*(m_i \mid t_i) \right) \exp( -\Lambda ),
\end{equation*}
where $\Lambda$ denotes the integral term $\Lambda = \int_{[0,T]} \lambda^*(\tau) \D\tau$.
%

\subsection{Causal Inference}
\label{sec:causalinference}

Causal effects are widely studied in the language of potential outcomes \citep[\textsc{Po},][]{neyman1923applications,rubin1978bayesian} or structural causal models \citep[\textsc{Scm},][]{pearl2009causality}. In this section, we briefly introduce both frameworks, as we use \textsc{Po}s to define causal queries formally and show their identifiability, while using \textsc{Scm}s to emphasize the distinction between probability distributions induced by different types of target causal queries.

\subsubsection{Potential Outcomes}

%
Let $A$ and $Y$ denote a treatment and an outcome variable. In the \textsc{Po} framework, the primitive building block is the potential outcome $Y[\tilde{a}]$, which is a random variable that represents the value of the outcome $Y$ under a treatment intervention $[A=\tilde{a}]$. The treatment intervention $[\tilde{a}]$ corresponds to the \textit{do-operator} $\doOperator(A=\tilde{a})$ in the \textsc{Scm} framework: $P(Y[\tilde{a}]) \equiv P(Y \mid \doOperator(A=\tilde{a}))$ \citep{pearl2009causality}.
%

\subsubsection{Observational, Interventional and Counterfactual Distributions}

\newcommand*{\DAGParent}{\operatorname{pa}}
For a set of variables $\mathbf{X} = \{X_k\}_{k=1}^K$, an \textsc{Scm} $\mathcal{M} = (\mathbf{S}, p(\mathbf{N}))$ consists of (i) a set of structural assignments $\mathbf{S} = \{X_k := f_k(\DAGParent(X_k), N_k)\}_{k=1}^K$, where $\DAGParent(\cdot)$ returns the parents of a given variable, and (ii) a distribution over noise variables $\mathbf{N} \sim p(\mathbf{N})$. A causal graph $\mathcal{G}$ is obtained by representing each variable $X_k$ as a node and drawing edges to $X_k$ from its parents $\DAGParent(X_k)$.
%
%
The \textsc{Scm} defines a generative process for $\mathbf{X}$ by sampling $\mathbf{N}$ from $p(\mathbf{N})$ and performing ancestral sampling over structural assignments $\mathbf{S}$, inducing an observational distribution $\mathbf{X} \sim p(\mathbf{X})$.
Each data point $\mathbf{x}^{(n)} = \{x_k^{(n)}\}_{k=1}^K$ in the observed data $ \mathcal{D} = \{\mathbf{x}^{(n)}\}_{n=1}^N$ is considered an i.i.d.~sample from the observational distribution.\looseness-1

An \emph{intervention} $\doOperator(X_k = \tilde{x}_k)$ is performed by removing the assignment $f_k(\cdot, \cdot)$ and setting $X_k$ to $\tilde{x}_k$. This yields an interventional \textsc{Scm} $\mathcal{M}_{\text{int}} = (\mathbf{S}_{\text{int}}, p(\mathbf{N}))$, inducing an interventional distribution: $p(\mathbf{X} \mid \doOperator(X_k = \tilde{x}_k)) \equiv p(\mathbf{X}[\tilde{x}_k])$.

In the context of an observed data point $\mathbf{x}^{(n)}$, we define a \emph{counterfactual} \textsc{Scm} by plugging in the individual's posterior noise distribution $p(\mathbf{N} \mid \mathbf{x}^{(n)})$ in place of the general (prior) noise distribution $p(\mathbf{N})$ and then updating the relevant structural assignment: $\mathcal{M}_{\text{cf}} = (\mathbf{S}_{\text{int}}, p(\mathbf{N} \mid \mathbf{x}^{(n)}))$. The resulting joint distribution $p(\mathbf{X} \mid \mathbf{x}^{(n)}, \doOperator(X_k = \tilde{x}_k)) \equiv p(\mathbf{X}[\tilde{x}_k] \mid \mathbf{x}^{(n)})$ is called the counterfactual distribution.

We categorize causal queries by the required joint distribution to answer them: (i) an interventional query requires access to the interventional distribution and (ii) a counterfactual query requires access to the counterfactual distribution. The key difference between the two queries is that a counterfactual query requires the posterior distribution of noise variables $p(\mathbf{N} \mid \mathbf{x}^{(n)})$ before performing the intervention, while the interventional query uses the noise prior $p(\mathbf{N})$.

\section{Problem Definition}
Consider an observational data set $\mathcal{D}$:
\begin{align}
    \label{eq:dataset}
    \mathcal{D} &= \big\{ \underbrace{\pi_{[0,T]}}_{\text{policy label}}, \underbrace{ \{(t_i, m_i)\}_{i=1}^{N_a} }_{\text{treatments } \mathbf{a}}, \underbrace{ \{(t_j, y_j)\}_{j=1}^{N_o} }_{\text{outcomes } \mathbf{o}} \big\},
\end{align}
in a period $[0,T]$. For notational ease, the data set is defined for a single patient. Our model can be trivially generalized to multiple patients, under exchangeability.

\begin{figure}[t]
\resizebox{\columnwidth}{!}{
\tikzset{mynode/.style={obs, minimum size=1.25cm}}
\tikzset{policy/.style={mynode, fill=red!10}}
\tikzset{action/.style={mynode, fill=blue!10}}
\tikzset{observation/.style={mynode, fill=yellow!10}}
\tikz{
    \node[text width=3cm] at (1.0, 0.25) {\huge{$\ldots$}};
    \node[observation] at (-7.2, 0.0)   (o1) {\huge$o_1$};
    \node[action] at (-5.55, -0.5)   (a1) {\huge$a_1$};
    \node[observation] at (-3.2, 1.4)   (o2) {\huge$o_2$};
    %
    \node[action] at (3.25, -0.5)   (a5) {\huge$a_i$};
    \node[observation] at (4.2, 1.6)   (o5) {\huge$o_j$};
    \node[action] at (6.1, -0.5)   (a6) {\LARGE$a_{i+1}$};
    \node[observation] at (7.5, 0.6)   (o6) {\LARGE$o_{j+1}$};
    \node[policy] at (-0.15, -2.8)   (pi) {\huge$\pi$};
\edge {o1} {a1}
\edge {o1,a1} {o2}
\edge {a5,a6,o5} {o6}
\edge {a5,o5} {a6}
\edge {a5} {o5}
\edge {pi} {a1,a5,a6}
\begin{scope}[on background layer]
    \draw (0, 0) node[inner sep=0]{\includegraphics[width=1.0\textwidth]{figures/figure2_plain_one_column_v2.pdf}};
    \draw (0, 0) node[inner sep=0, minimum height=7.0cm,minimum width=1.0\textwidth,fill=white,opacity=0.1]{};
 \end{scope}
}
}
\caption{The causal graph $\mathcal{G}$ assumes a sequential treatment--outcome setup in continuous time, where past treatments and outcomes have a causal effect on future treatments and outcomes. The causal effect of the policy $\pi$ on outcomes is fully mediated through treatments, i.e.~there are no direct edges between the policy $\pi$ and outcomes $\mathbf{o}$.}
\label{fig:causal_graph}
\end{figure}

A policy is a pair $(\pi_{[0,T]}, \lambda^*_{\pi}(t,m))$ that defines when and how treatments are applied, and is effectively determined by its treatment intensity function $\lambda^*_{\pi}(t,m)$. The policy label $\pi_{[0,T]}$ is assumed fixed for the period $[0,T]$ stated in the subscript, and it is assumed observed, while the corresponding intensity $\lambda^*_{\pi}(t,m)$ is unobserved. We assume that patients belong to different groups, and each group is characterized by a shared policy (treatment intensity). Background knowledge of having, e.g., different hospitals, countries, or environments in the observed data set implies distinct policies. In the absence of such information, each patient can be assumed to have their own policy.

 %

A treatment tuple $a_i=(t_i,m_i)$ consists of an arrival time $t_i \in [0,T]$ and a treatment mark (dosage) $m_i \in \mathbb{R}$. An outcome tuple $o_j=(t_j, y_j)$ consists of a measurement time $t_j \in [0,T]$ and an outcome value $y_j \in \mathbb{R}$. Treatment times $\mathbf{t_a}=\{t_i\}_{i=1}^{N_a}$ and outcome times $\mathbf{t_o}=\{t_j\}_{j=1}^{N_o}$ are irregularly sampled points on the interval $[0,T]$. The history $\mathcal{H}_{\leq t} = \{\pi_{\leq t}, \mathbf{a}_{\leq t}, \mathbf{o}_{\leq t}\}$ contains the information about the past policy $ \pi_{\leq t}$, past treatments $\mathbf{a}_{\leq t} = \{(t_i, m_i): t_{i} \leq t\}$ and past outcomes $\mathbf{o}_{\leq t} = \{(t_{j}, y_j): t_{j} \leq t\}$.

We observe a continuous-time process $\mathbf{Y}_{\leq T} = \{y(\tau): \tau \leq T\}$ as outcome tuples $\mathbf{o}$ measured at times $\mathbf{t_o} = \{t_j\}_{j=1}^{N_o}$. To answer causal queries, we model the potential outcome trajectory $\mathbf{Y}_{>\tilde{\tau}}[\tilde{\pi}_{>\tilde{\tau}}]$, under an intervened policy specified by $\tilde{\pi}_{>\tilde{\tau}}$, where the subscript emphasizes the period when a policy intervention takes place. When the intervention time $\tilde{\tau}$ is set to the end of the observation period $\tilde{\tau}=T$, we call the estimation task a \textit{policy intervention}, as its computation requires access to the interventional distribution (Fig. 1(b)):
\begin{align}
\label{eq:target_intervention}
    P(\mathbf{Y}_{>T}[\tilde{\pi}_{>T}] \mid \mathcal{H}_{\leq T}).
\end{align}
Also, we can set the intervention time $\tilde{\tau}$ to the start of the observation period $\tilde{\tau}=0$ and consider a hypothetical scenario under an alternative treatment policy specified by $\tilde{\pi}_{[0,T]}$. We call this estimation task a \textit{policy counterfactual}, as its computation requires access to the counterfactual distribution:
\begin{align}
\label{eq:target_counterfactual}
    P(\mathbf{Y}_{[0,T]}[\tilde{\pi}_{[0,T]}] \mid \mathcal{H}_{\leq T}).
\end{align}
The difference between a policy intervention and a policy counterfactual is illustrated in Figs.~\ref{fig:compare}~(b) and~(c).

\section{Causal Assumptions and Identifiability}

In this section, we first show that a policy intervention query, formalized in \cref{eq:target_intervention}, is equivalent to the potential outcome trajectory of a sequence of stochastic (conditional) interventions on treatments. Then, we show the latter is identifiable under causal assumptions, i.e., it can be estimated solely based on statistical terms \citep{pearl2009causality}.

\newcommand*{\obsPolicy}{\pi}
\newcommand*{\intPolicy}{\tilde{\pi}_{>T}}

We assume a sequential treatment--outcome setup where past treatments and outcomes may affect future events \citep{robins1986new,robins1987addendum}. We add the policy label $\pi$ to this setup, which has a direct causal effect on sequential treatments $\mathbf{a}$. The interplay between a policy label $\pi$, treatments $\mathbf{a}$, and outcomes $\mathbf{o}$ is illustrated in the causal graph $\mathcal{G}$ in \cref{fig:causal_graph}.
%
We make the standard causal assumptions of \emph{consistency} (Assumption 1) and \emph{no unobserved confounders} (\textsc{Nuc}, Assumption 2), and furthermore the continuous-time \textsc{Nuc} \citep[Assumption 3,][see formal definitions in \cref{sec:causal-assump}]{schulam2017reliable}. In words, the continuous-time \textsc{Nuc} states that treatments are assigned stochastically in continuous time, conditioned on the past history. In addition, we assume that the causal effect of the policy label $\pi$ on outcomes $\mathbf{o}$ is fully mediated through treatments $\mathbf{a}$, such that the causal graph $\mathcal{G}$ excludes direct edges from the policy label $\pi$ to the outcomes $\mathbf{o}$, stated formally as:

%

\textbf{Assumption 4: Fully-mediated policy effect.} Conditioned on the past history $\mathcal{H}_{\leq\tau}$, the causal effect of the policy specified by $\tilde{\pi}_{>\tau}$ on the outcome trajectory $\mathbf{Y}_{>\tau}$ is fully mediated through sequential treatments $\tilde{\mathbf{a}}_{>\tau}$: 
$$P(Y_{>\tau}[\tilde{\pi}_{>\tau}, \tilde{\mathbf{a}}_{>\tau}] \mid \mathcal{H}_{\leq \tau}) = P(Y_{>\tau}[\tilde{\mathbf{a}}_{>\tau}] \mid \mathcal{H}_{\leq \tau}).$$

Using Assumptions \{1,2,3,4\}, we inspect the potential outcome trajectory $\mathbf{Y}_{>T}[\intPolicy]$ at a discrete set of ordered query times $\mathbf{q}=\{q_1, \ldots, q_m\}$ (all $q_k > T$): $\mathbf{Y_q}[\tilde{\pi}_{>T}] = \{y(q_k)[\intPolicy]: q_k \in \mathbf{q}\}$ \citep{schulam2017reliable}. We factorize the outcome query $\mathbf{Y_q}[\intPolicy]$ in temporal order, and develop Theorem 1 below to reformulate it as the sequential estimation of treatments and outcomes:

%

%

%

\textbf{Theorem 1.} Under Assumptions \{1,2,3,4\}, the potential outcome query $\mathbf{Y_q}[\tilde{\pi}_{>T}]$ under a policy $\tilde{\pi}_{>T}$ is equivalent to the potential outcome query under a sequence of stochastic (conditional) interventions on treatments $\tilde{\mathbf{a}}_{>T}$:
\vspace{-1ex}
\begin{align}
    \label{eq:po_factorized}
    &P(\mathbf{Y_q}[\tilde{\pi}_{>T}] \mid \mathcal{H}_{\leq T}) = \sum_{\tilde{\mathbf{a}}_{>T}} \prod_{k=0}^{m-1} \\
    &\qquad\! P(\tilde{\mathbf{a}}_{[q_k, q_{k+1})}[\tilde{\pi}_{>T}] | \mathcal{H}_{\leq q_k}) \, P(Y_{q_{k+1}}[\tilde{\mathbf{a}}_{[q_k, q_{k+1})}] | \mathcal{H}_{\leq q_k}) , \nonumber
\end{align}
where $q_0 = T$, and $\tilde{\mathbf{a}}_{[q_{k}, q_{k+1})}$ denotes treatments in the interval $[q_{k}, q_{k+1})$ without outcome observations between consecutive query times. Here, the (whole) treatment sequence $\tilde{\mathbf{a}}_{>T}$ follows a distribution $p(\tilde{\mathbf{a}}_{>T}[\tilde{\pi}_{>T}])$, induced by the intervened policy label $\tilde{\pi}_{>T}$. The proof of Theorem 1 is given in \cref{sec:causal-iden}. Accordingly, the potential outcomes $\tilde{\mathbf{a}}_{[q_k, q_{k+1})}[\tilde{\pi}_{>T}]$ and $Y_{q_{k+1}}[\tilde{\mathbf{a}}_{[q_k, q_{k+1})}]$ can be identified under Assumptions \{1,2,3\}, using the following conditionals, both of which can be estimated with a statistical model \citep{schulam2017reliable,seedat2022continuous}:
\begin{align}
    \label{eq:stats_quantities}
    &P(\mathbf{Y_q}[\tilde{\pi}_{>T}] \mid \mathcal{H}_{\leq T}) = \sum_{\tilde{\mathbf{a}}_{>T}} \prod_{k=0}^{m-1} \\
    &\qquad\!\underbrace{P(\tilde{\mathbf{a}}_{[q_k, q_{k+1})} | \tilde{\pi}_{>T}, \mathcal{H}_{\leq q_k})}_{\text{Treatment Term}} \underbrace{P(Y_{q_{k+1}} | \tilde{\mathbf{a}}_{[q_k, q_{k+1})}, \mathcal{H}_{\leq q_k})}_{\text{Outcome Term}} . \nonumber
\end{align}
The identifiability result by \citet{schulam2017reliable} was limited to a fixed sequence of treatments. Theorem 1 and the identifiability result in \cref{eq:stats_quantities} generalize that result to a stochastic (conditional) intervention on a sequence of treatments, and one can recover the fixed sequence of treatments by assuming that the target density $p_{\tilde{\pi}}(\tilde{\mathbf{a}}_{>T})$ puts all probability on a single sequence of treatments. The identifiability of a policy counterfactual is more challenging and discussed in \cref{sec:inference}, since it requires functional assumptions related to the model definition (\cref{sec:joint-model}).

%
%

%

\section{Joint Treatment--Outcome Model}
\label{sec:joint-model}

To estimate both statistical terms in \cref{eq:stats_quantities}, (i) Treatment Term and (ii) Outcome Term, from observational data, we propose a joint treatment--outcome model, combining a marked point process and a conditional Gaussian process.

We encode conditional independence statements in the graph $\mathcal{G}$ by defining two dependent \textsc{Mpp}s with conditional intensity functions: (i) treatment intensity for a treatment $a=(t,m)$: $\lambda_{\pi}^*(t, m) = \lambda_{\pi}^*(t) p^*(m \mid t)$ and (ii) outcome intensity for an outcome $o=(t,y)$: $\lambda_o^*(t, y) = \lambda_o^*(t) p^*(y \mid t)$. The past history $\mathcal{H}_{<t} = \{ \pi_{<t}, \mathbf{a}_{<t}, \mathbf{o}_{<t} \}$ containing the information about the policy, past actions, and past outcomes is a valid history for both conditional intensity functions $\lambda_{\pi}^*(t, m)$ and $\lambda_o^*(t, y)$. The joint distribution for the observational data set $\mathcal{D}$ in \cref{eq:dataset} can be written in terms of treatment and outcome intensity functions:
\begin{equation*}
    p(\mathcal{D}) = \prod_{i=1}^I \lambda_{\pi}^*(t_i,m_i)
    \prod_{j=1}^J \lambda_o^*(t_j,y_j) \exp(-\Lambda),
\end{equation*}
with the integral term $\Lambda = \int_{[0,T]} \big(\lambda_{\pi}^*(\tau) + \lambda_{o}^*(\tau)\big) \D\tau$.

We further assume that the measurement times of the outcomes $\mathbf{t_o} = \{ t_j \}_{j=1}^{N_o}$ are given, which is valid for example when the data are collected through automated patient monitoring in healthcare. This assumption is equivalent to setting the outcome time intensity to an indicator function $\mathbbm{1}_{\mathbf{t_o}}(t)$:\footnote{The indicator function is: $\mathbbm{1}_{\mathbf{t_o}}(t) = \begin{cases}
      1, & \text{if}\ t \in \mathbf{t_o} \\
      0, & \text{otherwise}
    \end{cases}$}
$\lambda_o^*(t, y) = \mathbbm{1}_{\mathbf{t_o}}(t) p^*(y \mid t) = p^*(y \mid t)|_{t \in \mathbf{t_o}}$. Then, the joint distribution becomes
%
\begin{multline}
    p(\mathcal{D}) = \prod_{i=1}^I \underbrace{\lambda_{\pi}^*(t_i)  p^*_{\pi}(m_i \mid t_i)}_{\text{Treatment Intensity}}
    \prod_{j=1}^J \underbrace{p^*(y_j \mid t_j)}_{\text{Outcome Model}}|_{t_j \in \mathbf{t_o}} \\
    \times \exp(-\textstyle\int_{[0,T]} \lambda_{\pi}^*(\tau) \D\tau) .
    \label{eq:joint_intensity}
\end{multline}
%

\subsection{Treatment Intensity}
\label{sub:action}

%
We consider the treatment time intensity $\lambda^*_{\pi}(\tau)$ as the output of a square transformation of a latent function $g^*_{\pi}(\tau)$, which we model as the sum of a constant baseline $\beta_0$ and three time-dependent functions with \textsc{Gp} priors, $g_b, g^*_a, g^*_o \sim \mathcal{GP}$.
We assume the patients who follow the same treatment policy $\pi$ share the same treatment model, i.e., the same hyperparameters, but the intensity curves may differ because past treatments and outcomes are not the same.

The latent-state function $g_b(\tau)$ models the history-independent intensity. The regressive component $g^*_a(\tau)$ models the dependence on past treatments by taking the last $Q_a$ treatments as input and the regressive component $g^*_o(\tau)$ models the dependence on past outcomes by taking the last $Q_o$ outcomes as input. The treatment intensity $\lambda^*_{\pi}(\tau)$ is \looseness-1 %
%
\begin{equation}
    \label{eq:treatment_intensity}
    \lambda^*_{\pi}(\tau) = \big( \underbrace{\beta_0}_{\substack{\text{Poisson} \\ \text{Baseline}}} + \underbrace{g_b(\tau)}_{\substack{\textsc{Nhpp} \\ \text{Baseline}}} + \underbrace{g^*_a(\tau; \mathbf{a})}_{\substack{\text{Treatment} \\ \text{Effect}}} + \underbrace{g^*_o(\tau; \mathbf{o})}_{\substack{\text{Outcome} \\ \text{Effect}}} \big)^2 .
\end{equation}
%
%
%
The resulting treatment intensity extends the model proposed by \citet{liu2019nonparametric} with (i) additional baseline components $\beta_0$ and $g_b(\tau)$ and (ii) the functional dependence on marks.
%
Without regressive components $g^*_a(\tau)$ and $g^*_o(\tau)$, the treatment model becomes a non-homogeneous Poisson process (\textsc{Nhpp}), whose instantaneous intensity is independent of past events: $\lambda(\tau) = \smash{(\beta_0 + g_b(\tau))^2}$. If we further exclude the time-varying baseline $g_b(\tau)$, the model becomes a simple Poisson process with constant intensity. We model the treatment dosages (marks) by a \textsc{Gp}-prior: $m(\tau) \sim \mathcal{GP}$. The model definition is detailed in \cref{sec:treatment-details}.

\subsection{Outcome Model}

We model the outcome trajectory $\mathbf{Y} = \{y(\tau): \tau \in \mathbb{R}_{\geq 0}\}$ over time $\tau$ by a conditional \textsc{Gp} model, combining three independent components: (i) a baseline progression, (ii) a treatment response curve, and (iii) a noise variable \citep{schulam2017reliable,cheng2020patient,zhang2020errors}: %
\begin{equation}
    \label{eq:outcome}
    y(\tau) = \underbrace{f_b(\tau)}_{\text{Baseline}} + \underbrace{f_a(\tau; \mathbf{a})}_{\text{Treatment Response}} + \underbrace{\epsilon(\tau)}_{\text{Noise}},
\end{equation} %
with independent Gaussian noise $\epsilon(\tau) \sim \mathcal{N}(0,\sigma^2_{\epsilon})$.

\textbf{Baseline Progression.} This is modeled by a \textsc{Gp} prior on $f_b(\tau) \sim \mathcal{GP}$. \citet{cheng2020patient} proposed a sum of a squared exponential (\textsc{Se}) and a periodic kernel to model recurring patterns in heart rates. In our experiments, we model the baseline progression of blood glucose as a sum of a constant and a periodic kernel to capture daily blood glucose profiles of non-diabetic patients fluctuating around a constant baseline \citep{ashrafi2021computational}. We assume that the outcome baseline $f_b$ is patient-specific.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/figure3_v6.pdf}
    \hack{\vspace{-1ex}}
    \caption{The outcome model $f$ ({\color{red!80!white} red}) is the sum of baseline $f_b$ ({\color{olive} yellow}) and total response $f_a$, which adds up single treatment responses of different magnitude (3 {\color{blue!80!white} blue} lines). \looseness-1}
    \label{fig:treatment_effect}
    \hack{\vspace{-1ex}}
\end{figure}

\textbf{Treatment Response Model.} We model the treatment responses as additive, similar to \citet{cheng2020patient}: 
\begin{align}
    \label{eq:treatment_effect}
    f_a(\tau; \mathbf{a}) &= \sum_{a_i=(t_i,m_i) \in \mathbf{a}} f_m(m_i) f_t(\tau; t_i),
\end{align}
%
where the time-dependent response function $f_t \sim \mathcal{GP}$ represents the response `shape' and is shared across patients, and $f_m(m_i)$ is a patient-specific linear function that scales the magnitude of the response for the given treatment dosage value $m_i \in \mathbb{R}$, as commonly done in the literature \citep{cheng2020patient,zhang2020errors}. 
This means the effects of nearby treatments simply sum up as shown in \cref{fig:treatment_effect}.
The scaling function $f_m$ has patient-specific parameters that have hierarchical priors, to share information between patients.
For the response shape function $f_t$ we use an \textsc{Se} kernel, as it provides sufficient performance for our use-case (\citet{cheng2020patient} also propose an extension with a latent force model \citep{alvarez2009latent}).
The model definition is detailed in \cref{sec:outcome-details}.

\section{Inference}
\label{sec:inference}

\paragraph{Policy Intervention.} To model the policy intervention, we first fit the joint model to the observational data using variational inference (see \cref{sec:learning}), which gives us the (observational) SCM $\mathcal{M} = (\mathbf{S}, p(\mathbf{N}))$. An intervention $[\tilde{\pi}]$ on the policy results in an interventional \textsc{Scm}: $\mathcal{M}_{\text{int}} = (\mathbf{S}_{\text{int}}, p(\mathbf{N}))$. Following Theorem 1, this intervention is equivalent to a stochastic intervention on the sequence of treatments, where the treatments now follow the new policy $\tilde{\pi}$. In practice, this is modeled by replacing the observed treatment intensity $\lambda^*_{\pi}(\cdot)$ with the new interventional intensity $\lambda^*_{\tilde{\pi}}(\cdot)$, while keeping the outcome model the same.%


\paragraph{Policy Counterfactual.} The policy counterfactual is calculated in exactly the same way as the policy intervention, except that the generic noise term $p(\mathbf{N})$ is replaced by individual-specific noise $p(\mathbf{N} \mid \mathcal{D}^{(v)})$ that has been inferred from the observations for that individual $(v)$: 
%
$\mathcal{M}_{\text{cf}} = (\mathbf{S}_{\text{int}}, p(\mathbf{N} \mid \mathcal{D}^{(v)}))$.
In our model, the noise consists of two components, treatment and outcome noise: $\mathbf{N} = \{\mathcal{E}_a, \mathcal{E}_o\}$. The outcome noise $\mathcal{E}_o$ is defined in \cref{eq:outcome} and its posterior is available in closed form from the \textsc{Gp}.
%
The treatment noise $\mathcal{E}_a$ comprises noise associated with the sampling process of the treatments. In practice, we estimate the noise and condition the counterfactual sampling of the treatments with these estimates using a novel variant of the algorithm proposed by \citet{noorbakhsh2021counterfactual}, which we have extended to history-dependent point processes (see \cref{sssec:cf_algo}). 

\paragraph{Identifiability of the policy counterfactual.} The counterfactual trajectories involve two components: treatments and outcomes. The counterfactual \emph{treatments} are identifiable, as our algorithm satisfies the monotonicity assumption \citep{pearl2009causality, noorbakhsh2021counterfactual}. On the other hand, the counterfactual \emph{outcomes} are not guaranteed to be identifiable, because this would require identifiability of the baseline and treatment response separately, which is not guaranteed as they both are modeled non-parametrically.
%
To address this, we use priors that encourage the baseline (slow-changing) and the response functions (fast-changing) to learn different aspects of the data, and we empirically show that in practice the response function $f_a(\tau)$ (\cref{eq:treatment_effect}) and hence the counterfactual trajectory can be identified with good accuracy. The counterfactual algorithm and identifiability are further detailed in \cref{sssec:cf-id}.

\section{Experiments}

In this section, we validate that our model can estimate interventional and counterfactual outcome trajectories under policy interventions. The empirical validation is composed of two parts. First, on a \emph{real-world observational dataset}, we show the proposed model can learn clinically meaningful treatment response curves and treatment intensities that can handle time-varying confounding. Second, we evaluate our model on two causal inference tasks: (i) the policy intervention and (ii) the policy counterfactual. To evaluate the performance on interventional and counterfactual predictions, we set up a \emph{realistic semi-synthetic simulation} scenario, as the true causal effects are unknown for real-world observational data sets. To ensure a realistic simulation scenario, we use a subset of learned models from the real-world study as the ground-truth data generators. The study is reproducible and our implementation in GPflow \citep{GPflow2020multioutput} can be found at \url{https://github.com/caglar-hizli/modeling-policy-interventions}.

\subsection{Learning Treatment Intensities and Response Curves on Real-World Observational Data}
\label{subsec:exp-real-world}

\begin{figure*}[t]
    \hspace{-1cm}\includegraphics[width=1.1\linewidth]{figures/train_fit_d1_p8_fig3.pdf}
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    \caption{Estimated treatment--outcome model on the real-world meal--glucose data. \textbf{Top:} Glucose (outcome) measurements (black crosses), inferred baseline ({\color{olive}yellow}), and predicted glucose levels obtained by adding treatment responses, the baseline, and the noise ({\color{red}red}). The confidence intervals around the means refer to $\pm1$ standard deviation. We see that the increase in blood glucose is correctly predicted by the outcome model. \textbf{Bottom:} Treatment times and estimated intensities for the best model $\lambda_{ao}^*$ and the simple baseline $\lambda_b$. The baseline treatment model has a large meal intensity at times of the day when the patient usually eats. In addition, in the best treatment model, $\lambda_{ao}^*$, we see that the intensity of a new meal immediately after a previous meal decreases either directly through $g^*_a$ or indirectly through the increase in blood glucose represented by $g^*_o$. The intensities of the other models are shown in \cref{subsec:real_world_model}.}
    \label{fig:treatment_model_fit}
\end{figure*}

We first demonstrate that our model can learn clinically meaningful treatment intensities and response curves from a real-world observational dataset on physiological dynamics of blood glucose \citep{zhang2020errors,wyatt2021postprandial}. The experimental setup is further detailed in \cref{ssec:real-world}.

\textbf{Real-world dataset.} The dataset consists of treatment--outcome measurements of 14 non-diabetic patients over a 3-day period \citep{zhang2020errors}, corresponding to meals (treatments) and blood glucose measurements (outcomes). Patients record their meals in a meal diary and their blood glucose is measured by a monitoring device at regular time intervals. Meal ingredients are transformed into five nutrients: sugar, starch, protein, fiber, and fat. As meal dosage (mark), we preprocess nutrient covariates and use a single carbohydrate intake covariate equal to the sum of sugar and starch values, following \citet{ashrafi2021computational}.

\textbf{Causal Assumptions.} In the real-world dataset, the causal assumptions do \textbf{not} (exactly) hold and are not statistically testable. This is why (i) in this section, we perform only a \textit{statistical} analysis to show how our joint model works, and (ii) in \cref{ssec:semi}, we perform a \textit{causal} analysis on a semi-synthetic simulation study.

Assumption 2 states that an interventional meal has non-zero probability, which is likely to hold since we assume each patient follows their own diet (policy) and one patient's diet includes reasonable meal events that would have non-zero probability for the others. Assumption 3 does \emph{not} hold, since there can be unobserved processes, e.g., physical activity, which influence both meal times and daily glucose profiles.
However, the influence of confounding variables on blood glucose, apart from meals, is expected to be minor for non-diabetic individuals, as blood glucose is typically steady between meals \citep{ashrafi2021computational}.
Assumption 4 states that the policy effect is fully mediated through meals. 
For example, a policy that satisfies this is a dietary policy that dictates how the patient eats and in that way affects the blood glucose, but does not affect blood glucose in any other direct or indirect way. In \cref{ssec:semi}, we perform a causal analysis under such dietary policy interventions. As an example that violates this assumption, we could consider a more generic lifestyle intervention that includes aspects other than the diet, such as physical activity.

\textbf{Model.} The sequential meal--blood glucose data of a patient is modelled jointly, as detailed in Section \ref{sec:joint-model}. To show how the treatment intensity $\lambda^*(\tau)$ handles the time-varying confounding due to previous treatments and outcomes, we define five treatment intensities $\{\lambda_b, \lambda^*_{ba}, \lambda^*_{bo}, \lambda^*_{ao}, \lambda^*_{bao}\}$ for comparison.
In the most complex model $\lambda^*_{bao}$, the intensity of treatments depends on the baseline ($b$), previous treatments ($a$ for `action'), and previous outcomes ($o$); the simpler models have only some of these components as specified in their respective subscripts, see the functional forms in \cref{tab:testll}. 
%

\begin{table}
  \caption{Comparison of models for real-world data. The last column shows the test log-likelihood (\textsc{Tll}, higher is better; mean $\pm$ standard deviation) for the different models. Models are trained on the first 2 days of meal--glucose data. Day 3 is used to compute the \textsc{Tll}. %
  }
  \label{tab:testll}
  \centering
  \addtolength{\tabcolsep}{-3pt}
  \begin{tabular}{ccc}
    \toprule
    %
    %
    \textsc{Int\rlap{ensity}} & \textsc{Components} & \textsc{Tll} $\uparrow$ \\
    \midrule
    $\lambda_{b}$ & $\big(\beta_0 + g_{b}(\tau) \big)^2$ & $-13.3 \pm 0.5$ \\
    $\lambda_{ba}^*$ & $\big(\beta_0 + g_b(\tau) + g^*_a(\tau; \mathbf{a}) \big)^2$ & $-12.2 \pm 0.3$ \\
    $\lambda_{bo}^*$ & $\big(\beta_0 + g_b(\tau) + g^*_o(\tau; \mathbf{o}) \big)^2$ & $-11.0 \pm 0.3$ \\
    $\lambda_{ao}^*$ & $\big(\beta_0 + g^*_a(\tau; \mathbf{a}) + g^*_o(\tau; \mathbf{o}) \big)^2$ & $-10.7 \pm 0.4$ \\
    $\lambda_{bao}^*$ & $\big(\beta_0 + g_b(\tau) + g^*_a(\tau; \mathbf{a}) + g^*_o(\tau; \mathbf{o}) \big)^2$ & $-12.5 \pm 0.4$ \\
    \bottomrule
  \end{tabular}
\end{table}

\textbf{Results.} We show an example fit of the joint model for one patient in \cref{fig:treatment_model_fit}. The treatment- and outcome-dependent intensity $\lambda^*_{ao}$ (blue dashed line) correctly estimates that the probability of a meal event decreases (i) right after a new meal or (ii) with increasing blood glucose. This empirical finding suggests that functions $g^*_a$ and $g^*_o$ are useful in handling time-varying confounding due to past meal and glucose values.

%

%

We compare the different models in terms of the test log likelihood (\textsc{Tll}) for 14 patients in Table \ref{tab:testll}. We see that the simple history-independent intensity $\lambda_b(\tau)$ produces the lowest \textsc{Tll}. The treatment- and outcome-dependent intensity $\lambda_{ao}^*(\tau)$ produces the highest \textsc{Tll} mean, and slightly better results than the more complex intensity $\lambda_{bao}^*(\tau)$.

%


\colorlet{mylightblue}{blue!70!white}
\newcommand*{\citetablesup}[1]{{\color{mylightblue}$^{\textsc{(#1)}}$}}
\colorlet{mydarkblue}{blue!70!black}
\newcommand*{\ours}[1]{\textbf{\color{mydarkblue} \textsc{#1}}}
\newcommand*{\scm}[1]{$_{\text{#1}}$}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\begin{table*}[t]
  \footnotesize
  \caption{Causal tasks on semi-synthetic data: The \emph{observed} policy is $\pi_{[0,1d]} = \pi_A$, and we report mean squared error (\textsc{Mse}, lower is better) for observational $[\tilde{\pi}_{>1d} = \pi_A]$ and interventional $[\tilde{\pi}_{>1d} = {\color{red}\pi_B}]$ queries as well as for the policy counterfactual $[\tilde{\pi}_{\color{red}[0,1d]} = {\color{red}\pi_B}]$. The best results are \textbf{bolded}. Methods developed by us are highlighted in {\color{mydarkblue} \textbf{blue}}.}
  \label{tab:intervention}
  \label{tab:counterfactual}
  \centering
  \newcommand*{\nhpp}{\textsc{Nhpp}\citetablesup{L15}}
  \newcommand*{\gammap}{Gamma\citetablesup{H21}}
  \newcommand*{\paramSchulam}{Param.\citetablesup{S17}}
  \newcommand*{\paramHua}{Param.\citetablesup{H21}}
  \sisetup{detect-weight, separate-uncertainty=true, add-integer-zero=false}
  \begin{tabular}{lllS[table-format=1.2+-1.2]S[table-format=1.2+-1.2]lS[table-format=1.2+-1.2]}
    \toprule
    %
    %
    & & \multicolumn{3}{c}{\textsc{Query} (\textsc{Mse} $\downarrow$)} & \multicolumn{2}{c}{\textsc{Query} (\textsc{Mse} $\downarrow$)} \\
    \cmidrule(lr){3-5}
    \cmidrule(lr){6-7}
    \multirow{2}{*}{\parbox{1cm}{\textsc{Treatment Model}}} & \multirow{2}{*}{\parbox{1cm}{\textsc{Response Model}}} & 
    \multirow{2}{*}{$\mathcal{M}_{\textsc{Scm}}$} & {\textsc{Observational}} & 
    {\textsc{Interventional}} &
    \multirow{2}{*}{$\mathcal{M}_{\textsc{Scm}}$} & {\textsc{Counterfactual}}
    \\
     & & & {$[\tilde{\pi}_{>1d} = \pi_{A}]$} & {$[\tilde{\pi}_{>1d} = {\color{red}\pi_{B}}]$} & & {$[\tilde{\pi}_{\color{red}[0,1d]} = {\color{red}\pi_{B}}]$} \\
    \midrule
    \gammap      & \paramHua     & H21\scm{int}          &     .50+-.02 &     .50 \pm .02 & H21\scm{cf}          &     .49+-.02 \\
    \gammap      & \ours{Gp}     & \textsc{Ab1}\scm{int} &     .30+-.02 &     .30 \pm .01 & \textsc{Ab1}\scm{cf} &     .21+-.01 \\
    \nhpp        & \paramSchulam & \textsc{Ab2}\scm{int} &     .97+-.03 &    1.00 \pm .03 & \textsc{Ab2}\scm{cf} &     .59+-.02 \\
    \nhpp        & \ours{Gp}     & \textsc{Ab3}\scm{int} &     .34+-.02 &     .32 \pm .01 & \textsc{Ab3}\scm{cf} &     .23+-.01 \\
    \ours{Gp-pp} & \paramHua     & \textsc{Ab4}\scm{int} &     .46+-.01 &     .46 \pm .01 & \textsc{Ab4}\scm{cf} &     .45+-.02 \\
    \ours{Gp-pp} & \paramSchulam & \textsc{Ab5}\scm{int} &     .96+-.03 &    1.00 \pm .03 & \textsc{Ab5}\scm{cf} &     .56+-.02 \\
    \ours{Gp-pp} & \ours{Gp}     & \ours{Our}\scm{obs}   & \bf .19+-.01 &     .52 \pm .02 & \ours{Our}\scm{obs}  &     .82+-.03 \\
    \ours{Gp-pp} & \ours{Gp}     & \ours{Our}\scm{int}   & \bf .19+-.01 & \bf .20 \pm .01 & \ours{Our}\scm{int}  &     .71+-.03 \\
    \ours{Gp-pp} & \ours{Gp}     & \ours{Our}\scm{cf}    & \bf .19+-.01 & \bf .20 \pm .01 & \ours{Our}\scm{cf}   & \bf .14+-.01 \\
    \bottomrule
  \end{tabular}
\end{table*}

\subsection{Causal Tasks on Semi-Synthetic Data}
\label{ssec:semi}

In this section, we set up a semi-synthetic simulation study to demonstrate the ability of the proposed model to answer interventional and counterfactual queries resulting from an intervention on the treatment policy. Due to space constraints, the experimental setup is detailed in \cref{ssec:semi-synth}.

%

\textbf{Simulator.} We obtain the ground-truth simulator by fitting our joint model to the meal--glucose data set, as discussed in Section \ref{subsec:exp-real-world}. To be able to assess the sequential causal inference tasks, we have to include both sources of time-varying confounding. Therefore, we select as the ground-truth meal simulator the intensity that depends on both meal and glucose histories: $\lambda^{*}_{\pi} \sim \lambda^*_{ao}$.

%

\newcommand*{\piA}{{\color{blue}\pi_A}}
\newcommand*{\piB}{{\color{red}\pi_B}}
\textbf{Semi-synthetic dataset.} The ground-truth simulator is used to simulate samples from observational, interventional and counterfactual distributions of each patient $(v)$. Simulated patients are divided into (i) two policy groups $\{\piA, \piB\}$ representing different diets and (ii) three patient groups with distinct baseline and response functions, enabling individualization among patients. The meal simulators of two diets correspond to learned intensity functions of two real-world patients. The glucose simulators of three groups are learned from three real-world patients.

\newcommand*{\oneday}{\SI{1}{\day}}
For the observational data set, we simulate 1-day long meal--glucose time-series for 50 patients: $\mathcal{D} = \{\mathcal{D}^{(v)}\}_{v=1}^{50}$. For the interventional data set, we sample the next day of each patient under the specified policy intervention $[\tilde{\pi}_{>1d}]$. For the counterfactual data set, we condition on the observed data $\mathcal{D}^{(v)}$ for each patient and sample a hypothetical first day under a policy intervention $[\tilde{\pi}_{[0,1d]}]$, using the noise posteriors. We train all models on the observational dataset, and use interventional and counterfactual datasets for testing.

%


\textbf{Benchmarks.} First, we compare the proposed model with a parametric joint model \citep[\textsc{H21},][]{hua2021personalized}, which uses a renewal process with a parametric Gamma-shaped trigger function as the treatment model, and a linear mixed effects function as the outcome model. Next, we create ablations with different treatment and outcome model combinations, since other existing methods do not model treatments. With ablations having different treatment intensities, we measure the impact of having a flexible treatment intensity that can handle complex time-varying confounding scenarios. With ablations having different outcome models, we measure the impact of predicting the glucose trajectory well. The ablation \textsc{Ab1} combines the Gamma-based treatment intensity with our \textsc{Gp}-response model. Ablations \textsc{Ab2} and \textsc{Ab3} combine a history-independent treatment model \citep[\textsc{Nhpp},][\citetablesup{L15}]{lloyd2015variational} with (i) a parametric response model proposed by \citet[\citetablesup{S17}]{schulam2017reliable} and (ii) our \textsc{Gp}-response model. Ablations \textsc{Ab4} and \textsc{Ab5} combine our flexible treatment intensity (\textsc{Gp-pp}) with two parametric response models proposed by \citet[\citetablesup{H21}]{hua2021personalized} and \citet[\citetablesup{S17}]{schulam2017reliable}.

The columns $\mathcal{M}_{\textsc{Scm}}$ in \cref{tab:intervention} specify the combination of (i) a joint model identifier $\mathcal{M}$, e.g., \textsc{Our}, and (ii) the target distribution of the \textsc{Scm} stated as a subscript: $(\cdot)$\scm{obs} for observational, $(\cdot)$\scm{int} for interventional, and $(\cdot)$\scm{cf} for counterfactual. Similar to \citet{schulam2017reliable}, we use our own observational model (\textsc{Our}$_\text{obs}$) as another baseline in the interventional task. In the counterfactual task, we use both our observational (\textsc{Our}$_\text{obs}$) and interventional model (\textsc{Our}$_\text{int}$) as baselines. Our counterfactual model is denoted by \textsc{Our}$_\text{cf}$. To give our baseline and ablation models the most strength, we use their interventional version, ($\cdot$)\scm{int}, for estimating the interventional query and their counterfactual version, $(\cdot)$\scm{cf}, for estimating the counterfactual query.

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\textbf{Metric.} We report the mean squared error (\textsc{Mse}) between ground-truth and estimated glucose trajectories under the interventional and counterfactual distributions, over all patients and all measurement times. To obtain estimated trajectories comparable to the ground-truth trajectories, we fix the noise variables of the point process (meal) sampling algorithm between the ground-truth simulator and each estimated model. Each experiment is repeated 10 times. We report mean and standard deviation of the \textsc{Mse} metric.

\iffalse
\begin{table}
  \caption{\textsc{Mse} results for the policy counterfactual $[\tilde{\pi}_{[0,1d]} = \pi_B]$. The observed policy is $\pi_{[0,1d]} = \pi_A$. {\color{mydarkblue} \textbf{Blue}} represents methods developed by us.}
  \label{tab:counterfactual}
  \centering
  \footnotesize
  \begin{tabular}{lllc}
    \toprule
    %
    %
    \multirow{3}{*}{$\mathcal{M}_{\textsc{Scm}}$} & 
    \multirow{3}{*}{\parbox{1cm}{\textsc{Treat\rlap{ment} Model}}} & 
    \multirow{3}{*}{\parbox{1cm}{\textsc{Resp\rlap{onse} Model}}} & \textsc{Query} (\textsc{Mse} $\downarrow$) \\
    \cmidrule(r){4-4}
     &  & & {\tiny \textsc{Counterfactual}} \\
    %
     & & & $[\tilde{\pi}_{[0,1d]} = \pi_{B}]$ \\
    %
    %
    \midrule
    H21\scm{cf} & Gamma\citetablesup{H21} & Param.\citetablesup{H21} & $.51 \pm .02$ \\
    \textsc{Ab1}\scm{cf} & Gamma\citetablesup{H21} & \ours{Gp} & $.23 \pm .01$ \\
    \textsc{Ab2}\scm{cf} & \textsc{Nhpp}\citetablesup{L15} & Param.\citetablesup{S17} & $ .60 \pm .02 $ \\
    \textsc{Ab3}\scm{cf} & \textsc{Nhpp}\citetablesup{L15} & \ours{Gp} & $ .25 \pm .01 $ \\
    \textsc{Ab4}\scm{cf} & \ours{Gp-pp} & Param.\citetablesup{H21} & $.46 \pm .02$ \\
    \textsc{Ab5}\scm{cf} & \ours{Gp-pp} & Param.\citetablesup{S17} & $.57 \pm .02$ \\
    \ours{Our}\scm{obs} & \ours{Gp-pp} & \ours{Gp} & $ .86 \pm .04 $ \\
    \ours{Our}\scm{int} & \ours{Gp-pp} & \ours{Gp} & $ .71 \pm .03 $   \\
    \ours{Our}\scm{cf} & \ours{Gp-pp} & \ours{Gp} & $ \mathbf{.15 \pm .01} $ \\
    \bottomrule
  \end{tabular}
\end{table}
\fi

\textbf{Policy Intervention.} We estimate the interventional query: What will happen if patient $(v)$ with the diet $\pi^{(v)} = \piA$ will continue for the next day in the future, adopting another patient's diet $\piB$? Following \cref{eq:target_intervention}, the causal query for this task is formalized as the interventional query: \[ P(\mathbf{Y}^{(v)}_{>1d}[\tilde{\pi}_{>1d} = \piB] \mid \pi_{[0,1d]}=\piA, \mathcal{H}^{(v)}_{\leq 1d}). \]
\textsc{Mse} results are shown in Table \ref{tab:intervention}. We see that the interventional model \textsc{Our}$_{\text{int}}$ is able to estimate observational and interventional trajectories with low error when the intervention policy is (i) the same as the observed policy $[\tilde{\pi}_{>1d} = \piA]$ and (ii) different from the observed policy $[\tilde{\pi}_{>1d} = \piB]$, while the observational model \textsc{Our}$_{\text{obs}}$ fails in the latter case. This is because \textsc{Our}$_{\text{obs}}$ can only answer a statistical query of the following form: Observing the history of patient $(v)$, how will the patient state progress for the next day, $P(\mathbf{Y}^{(v)}_{>1d} \mid \pi_{[0,1d]}=\piA, \mathcal{H}^{(v)}_{\leq 1d})$? Furthermore, our empirical findings suggest that simplistic models with parametric glucose responses (Param.\citetablesup{S17,H21}) perform badly, even when they target the interventional distribution.

\textbf{Policy Counterfactual.} We estimate the counterfactual query: What \emph{would have} happened if patient $(v)$ with the diet $\pi^{(v)} = \piA$ had followed another patient's diet $\piB$ in the observation period $\color{red}[0,1d]$? Following \cref{eq:target_counterfactual}, the causal query for this task is formalized as the counterfactual \[ P(\mathbf{Y}^{(v)}_{\leq 1d}[\tilde{\pi}_{\color{red}[0,1d]} = \piB] \mid \pi_{[0,1d]}=\piA, \mathcal{H}^{(v)}_{\leq 1d}) . \] 
\textsc{Mse} results are shown in the last column of Table \ref{tab:counterfactual}. We see that the interventional model \textsc{Our}$_{\text{int}}$ fails to estimate counterfactual trajectories, as it does not take into account the noise posterior of each patient. On the other hand, the counterfactual model \textsc{Our}$_{\text{cf}}$ accurately samples counterfactual trajectories and has the smallest error of the methods considered.

\section{Discussion}

To study what happens if the (possibly implicit) treatment policy of one individual (hospital, unit, country, \dots) is or had been adopted by another individual, we proposed a model that jointly considers sequences of treatments and outcomes of each individual. Theoretically, we showed that an intervention on a treatment policy is equivalent to a sequence of stochastic interventions on treatments, whose potential outcomes can be estimated from observational data with the joint model. In a real-world scenario, we demonstrated that our non-parametric model can be learned from observational sequences of treatments and outcomes, and it can handle time-varying confounding in continuous time. In a semi-synthetic experiment, we demonstrated that the joint model can answer causal queries about the interventional and counterfactual distributions of the outcome after an intervention on the treatment policy.

\subsection{Limitations and Future Work}

\paragraph{Modeling Limitations.} The main limitation of the proposed outcome model is scalability, as it is not trivial to use inducing point approximations for the current `time-marked' treatment response function. This could be improved in future work, e.g., by clever inducing point selections. Furthermore, we considered treatment responses to be additive, which does not allow for modeling interactions of nearby treatments. This could be improved by integrating more sophisticated kernels into the treatment response function.

The thinning algorithm for sampling the point process is sequential and known to be slow, which can raise a challenge in using our method for downstream tasks such as optimizing the policy by a model-based reinforcement learning algorithm. It could be possible to adapt an inverse sampling method with $\mathcal{O}(1)$ time complexity \citep{rasmussen2011temporal}, but this would require a completely different treatment model definition as in \citet{schur2020fast}, whose applicability would need to be studied separately.

\paragraph{Causal Assumptions.}
For real-world observational datasets, our causal assumptions do not necessarily hold, in which case our method should not be used for \emph{causal} analysis (the model may still be useful for statistical analysis).
For example, the violation of the \textsc{Nuc} assumption would result in an error in the causal effect estimates due to the unblocked back-door paths, whose magnitude depends on the size of the violation.
An interesting future direction is to extend existing sensitivity analysis methods \citep{robins2000sensitivity} in order to estimate the size of the error in causal effects of continuous-time treatment sequences.

%
%

%
%
%
%
%
%

%

%

%

%
%
%
%
%
%

%
%
%
%
%
%
%

%

%

%

%

%

